LazyLLM: Dynamic Token Pruning for Efficient Long Context LLM Inference

The inference of transformer-based large language models consists of two sequential stages: 1) a prefilling stage to compute the KV cache of prompts and generate the first token, and 2) a decoding stage to generate subsequent tokens. For long prompts, the KV cache must be computed for all tokens during the prefilling stage, which can significantly increase the time needed to generate the first token. Consequently, the prefilling stage may become a bottleneck in the generation process. An open question remains whether all prompt tokens are essential for generating the first token. To answer this, we introduce a novel method, LazyLLM, that selectively computes the KV for tokens important for the next token prediction in both the prefilling and decoding stages. Contrary to static pruning approaches that prune the prompt at once, LazyLLM allows language models to dynamically select different subsets of tokens from the context in different generation steps, even though they might be pruned in previous steps. Extensive experiments on standard datasets across various tasks demonstrate that LazyLLM is a generic method that can be seamlessly integrated with existing language models to significantly accelerate the generation without fine-tuning. For instance, in the multi-document question-answering task, LazyLLM accelerates the prefilling stage of the LLama 2 7B model by 2.34x while maintaining accuracy.

==> tables/tasks_results_v1_lock.tex <==
\begin{table*}[h!]
    \begin{center}
    \begin{scriptsize}
    \begin{sc} 
    \centering
    \begin{tabular}{c|cccc}
    \Xhline{1.0pt}  
    Model & Tasks & Method & Score & TTFT Speedup ($\times$)\\
    \hline
    \multirow{30}{*}{\makecell{Llama2}} & \multirow{5}{*}{Single-Document QA} & Baseline & $25.79$ & $1.00$\\
    &  & Random Token Drop & $20.05$ & $1.20$ \\
    &  & Static Token Pruning & $21.89$ & $1.18$ \\
    &  & Prompt Compression & $22.88$ & $0.12$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{25.59}$ & $\mathbf{1.36}$ \\ \cline{2-5}
     & \multirow{5}{*}{Multi-Document QA} & Baseline & $22.43$ & $1.00$ \\
     &  & Random Token Drop & $16.77$ & $1.19$ \\
     &  & Static Token Pruning & $19.93$ & $2.16$ \\
     &  & Prompt Compression & $8.42$ & $0.13$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{22.31}$ & $\mathbf{2.34}$ \\ \cline{2-5}
     & \multirow{5}{*}{Summarization} & Baseline & $24.65$ & $1.00$ \\
     &  & Random Token Drop & $24.39$ & $1.39$ \\
     &  & Static Token Pruning & $24.59$ & $1.33$ \\
     &  & Prompt Compression & $25.16$ & $0.12$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{24.75}$ & $\mathbf{1.46}$ \\ \cline{2-5}
     & \multirow{5}{*}{Few-shot Learning} & Baseline & $62.90$ & $1.00$ \\
     &  & Random Token Drop & $53.93$ & $1.19$ \\
     &  & Static Token Pruning & $56.54$ & $2.16$ \\
     &  & Prompt Compression & $24.18$ & $0.10$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{62.81}$ & $\mathbf{2.19}$ \\ \cline{2-5}
     & \multirow{5}{*}{Synthetic} & Baseline & $4.97$ & $1.00$ \\
     &  & Random Token Drop & $3.57$ & $1.18$ \\
     &  & Static Token Pruning & $2.81$ & $2.15$ \\
     &  & Prompt Compression & $3.20$ & $0.12$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{4.98}$ & $\mathbf{2.89}$ \\ \cline{2-5}
     & \multirow{5}{*}{Code Completion} & Baseline & $55.18$ & $1.00$ \\
     &  & Random Token Drop & $44.92$ & $1.23$ \\
     &  & Static Token Pruning & $37.51$ & $1.84$ \\
     &  & Prompt Compression & $17.45$ & $0.49$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{53.30}$ &  $\mathbf{1.94}$ \\ \cline{1-5}
     
     \multirow{30}{*}{\makecell{XGen}} & \multirow{5}{*}{Single-Document QA} & Baseline & $25.19$ & $1.00$ \\
     &  & Random Token Drop & $18.32$ & $1.58$ \\
     &  & Static Token Pruning & $19.30$ & $1.61$ \\
     &  & Prompt Compression & $15.31$ & $0.20$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{25.00}$ & $\mathbf{1.96}$ \\ \cline{2-5}
     & \multirow{5}{*}{Multi-Document QA} & Baseline & $20.71$ & $1.00$ \\
     &  & Random Token Drop & $14.86$ & $1.37$ \\
     &  & Static Token Pruning & $17.23$ & $2.11$ \\
     &  & Prompt Compression & $11.56$ & $0.19$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{20.68}$ & $\mathbf{2.65}$ \\ \cline{2-5}
     & \multirow{5}{*}{Summarization} & Baseline & $24.85$ & $1.00$ \\
     &  & Random Token Drop & $24.47$ & $1.70$ \\
     &  & Static Token Pruning & $24.46$ & $1.65$ \\
     &  & Prompt Compression & $24.57$ & $0.17$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{24.74}$ & $\mathbf{1.91}$ \\ \cline{2-5}
     & \multirow{5}{*}{Few-shot Learning} & Baseline & $56.40$ & $1.00$ \\
     &  & Random Token Drop & $46.35$ & $1.62$ \\
     &  & Static Token Pruning & $51.93$ & $3.17$ \\
     &  & Prompt Compression & $23.72$ & $0.15$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{56.12}$ & $\mathbf{3.42}$ \\ \cline{2-5}
     & \multirow{5}{*}{Synthetic} & Baseline & $5.40$ & $1.00$ \\
     &  & Random Token Drop & $2.53$ & $1.13$ \\
     &  & Static Token Pruning & $3.00$ & $4.14$ \\
     &  & Prompt Compression & $1.42$ & $0.17$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{5.66}$ & $\mathbf{4.77}$ \\ \cline{2-5}
     & \multirow{5}{*}{Code Completion} & Baseline & $36.49$ & $1.00$ \\
     &  & Random Token Drop & $32.34$ & $1.57$ \\
     &  & Static Token Pruning & $32.27$ & $2.97$ \\
     &  & Prompt Compression & $11.38$ & $0.69$ \\
     &  & \emph{LazyLLM (Ours)} & $\mathbf{36.47}$ & $\mathbf{3.47}$ \\ \cline{2-5}
    \Xhline{1.0pt}
    \end{tabular}
\end{sc}
\end{scriptsize}
    \caption{Comparisons of \ttft speedup \vs accuracy on various tasks. Without requiring any training/finetuning, \methodname consistently achieves better \ttft speedup with negligible accuracy drop.
    \label{tab:tasks_results}
    \end{center}
\end{table*}

